Attribute-Guided Multi-Level Attention Network for Fine-Grained Fashion Retrieval

Fine-grained fashion retrieval searches for items that share a similar attribute with the query image. Most existing methods use a pre-trained feature extractor (e.g., ResNet 50) to capture image representations. However, a pre-trained feature backbone is typically trained for image classification and object detection, which are fundamentally different tasks from fine-grained fashion retrieval. Therefore, existing methods suffer from a feature gap problem when directly using the pre-trained backbone for fine-tuning. To solve this problem, we introduce an attribute-guided multi-level attention network (AG-MAN). Specifically, we first enhance the pre-trained feature extractor to capture multi-level image embedding, thereby enriching the low-level features within these representations. Then, we propose a classification scheme where images with the same attribute, albeit with different values, are categorized into the same class. This can further alleviate the feature gap problem by perturbing object-centric feature learning. Moreover, we propose an improved attribute-guided attention module for extracting more accurate attribute-specific representations. Our model consistently outperforms existing attention based methods when assessed on the FashionAI (62.8788% in MAP), DeepFashion (8.9804% in MAP), and Zappos50k datasets (93.32% in Prediction accuracy). Especially, ours improves the most typical ASENet_V2 model by 2.12%, 0.31%, and 0.78% points in FashionAI, DeepFashion, and Zappos50k datasets, respectively. The source code is available in https://github.com/Dr-LingXiao/AG-MAN.

==> sec/2_relatedWork.tex <==
\section{Related work}
\label{sec:Related_work}

\subsection{Fashion retrieval}

As fashion recommendations become a trending research topic, fashion retrieval also attracts more attention~\cite{Gajic_CVPR_18,Zhao_CVPR_17,Han_ACMMultimedia_17,Ji_ACMMultimedia_17,Ibrahimi_ICCV_19,Sharma_WACV_21,Liu_ACMMM_21,Naka_ICMR_22, Islam_MM_23, Suzuki_ICMR_23}. Ji {\it et al.}~\cite{Ji_ACMMultimedia_17} leveraged detailed label information from e-commerce websites to improve cross-domain retrieval. This aided the attention mechanism in pinpointing clothing within complex scenes, facilitating in-shop retrieval based on the extracted clothing features. Han {\it et al.}~\cite{Han_ACMMultimedia_17} employed a bi-directional long short-term memory (Bi-LSTM) network to recommend an item for the given incomplete outfit in the fashion compatibility task. Subsequently, the advancement of the attention mechanism bolstered the models' capacity to understand context and witnessed widespread integration into computer systems~\cite{Woo_ECCV_18,Qiao_AAAI_18,Chen_ICCV_21,Vaswani_CVPR_21} and recommendation systems~\cite{Zhou_SIGKDD_18,Tay_SIGKDD_18,Liu_IS_21}.
Wang {\it et al.}~\cite{Wang_VCIP_17} used a self-guided attention module to autonomously capture clothing features without relying on external landmark annotations. Nevertheless, they primarily concentrated on the broader resemblance of attire, falling short of the requirements for fine-grained retrieval. To address this issue, several fine-grained fashion retrieval methods have been proposed~\cite{Veit_CVPR_17,Ma_AAAI_20,Wan_ETAI_22,Yan_ICME_22}. In~\cite{Veit_CVPR_17}, they learned an embedding space and used a fixed mask to select relevant dimensions of the embedding space based on a specified attribute. The masked embedding was adopted for final loss calculation. Different from it, Ma {\it et al.}~\cite{Ma_AAAI_20} proposed to acquire distinct embedding spaces tailored to specific attributes, rather than relying on a single and unified embedding space. To clarify, they evaluated the nuanced similarity within each corresponding feature space. Wan {\it et al.}~\cite{Wan_ETAI_22} presented a similar network architecture. They believed that the concurrent acquisition and integration of spatial and channel attention features are effective, with the exception of the sequential learning employed within the attention modules. Yan {\it et al.}~\cite{Yan_ICME_22} employed iterative learning strategies to this task. Xiao {\it et al.}~\cite{xiao_MIPR_23} employed a contrastive learning method for solving the multi-view problem~\cite{xiao_MIPR_23}. Jiao {\it et al.}~\cite{Jiao_ECCV_22} incorporated different supervisions at both instance and cluster level for more accurate fine-grained fashion retrieval.
However, they often overlooked the feature gap issue.




\subsection{Attention mechanism}

The attention mechanism witnessed a significant traction and has shown remarkable effectiveness in a variety of research domains, encompassing fields such as computer vision~\cite{Woo_ECCV_18,Zhao_CVPR_20,Niu_Neurocom_21,Li_AI_21,Hou_CVPR_21} and natural language processing~\cite{Vaswani_NIPS_17,Galassi_IEEE-NNLS_20,Sood_NIPS_20}. At its core, the attention mechanism can be understood as a method that allocates more weights towards the most relevant parts of the input data. 

In the fashion retrieval field, attention mechanisms are also very important because using a fixed region of interest for a specified attribute across all of the images is not optimal due to the diverse nature of fashion images, which often feature complex backgrounds, pose variations, and other factors. Consequently, attention mechanism is commonly used in the fashion domain~\cite{Ji_ACMMultimedia_17,Wang_VCIP_17,Han_ICCV_17,Ak_CVPR_18,Ak_WACV_18,Ma_AAAI_20}. For instance, Ak {\it et al.}~\cite{Ak_WACV_18} leveraged prior knowledge of garment construction to pinpoint the precise components of clothing. Nevertheless, their methodology was confined to upper-body clothing, restricting its broader applicability. Wang {\it et al.}~\cite{Wang_VCIP_17} proposed incorporating channel attention mechanisms into a fully convolutional network. Ji {\it et al.}~\cite{Ji_ACMMultimedia_17} employed attributes to enhance attention modeling. In~\cite{Ma_AAAI_20}, they introduced two attribute-guided attention mechanisms that used a specific attribute as auxiliary input alongside the given image. The suggested attention modules have successfully discerned patterns associated with the specified attribute under the directive of that attribute. Wan {\it et al.}~\cite{Wan_ETAI_22} improved existing attribute attention modules by fusing the spatial and channel attention information. Yan {\it et al.}~\cite{Yan_ICME_22} enhanced attribute localization accuracy through iterative refinement of the attention module. In contrast to existing methods, we theoretically analyze the feature gap problem in current fine-grained fashion retrieval methods and introduce a more powerful attention network for solving the problem and achieving more accurate fine-grained fashion retrieval.  

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.
